BinCoFer: Three-Stage Purification for Effective C/C++ Binary Third-Party Library Detection

Third-party libraries (TPL) are becoming increasingly popular to achieve efficient and concise software development. However, unregulated use of TPL will introduce legal and security issues in software development. Consequently, some studies have attempted to detect the reuse of TPLs in target programs by constructing a feature repository. Most of the works require access to the source code of TPLs, while the others suffer from redundancy in the repository, low detection efficiency, and difficulties in detecting partially referenced third-party libraries. Therefore, we introduce BinCoFer, a tool designed for detecting TPLs reused in binary programs. We leverage the work of binary code similarity detection(BCSD) to extract binary-format TPL features, making it suitable for scenarios where the source code of TPLs is inaccessible. BinCoFer employs a novel three-stage purification strategy to mitigate feature repository redundancy by highlighting core functions and extracting function-level features, making it applicable to scenarios of partial reuse of TPLs. We have observed that directly using similarity threshold to determine the reuse between two binary functions is inaccurate, a problem that previous work has not addressed. Thus we design a method that uses weight to aggregate the similarity between functions in the target binary and core functions to ultimately judge the reuse situation with high frequency. To examine the ability of BinCoFer, we compiled a dataset on ArchLinux and conduct comparative experiments on it with other four most related works (i.e., ModX, B2SFinder, LibAM and BinaryAI)...

==> CodeStyle.tex <==

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\lstset{ %
 backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
 basicstyle=\footnotesize,        % the size of the fonts that are used for the code
 breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
 breaklines=true,                 % sets automatic line breaking
 captionpos=bl,                    % sets the caption-position to bottom
 commentstyle=\color{mygreen},    % comment style
 deletekeywords={...},            % if you want to delete keywords from the given language
 escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
 extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
 frame=single,                    % adds a frame around the code
 keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
 keywordstyle=\color{blue},       % keyword style
 language=Java,                 % the language of the code
 morekeywords={*,...},            % if you want to add more keywords to the set
 numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
 numbersep=5pt,                   % how far the line-numbers are from the code
 numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
 rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
 showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
 showstringspaces=false,          % underline spaces within strings only
 showtabs=false,                  % show tabs within strings adding particular underscores
 stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
 stringstyle=\color{orange},     % string literal style
 tabsize=2,
 xleftmargin=2em,
 xrightmargin=2em,
}
